Compiler Directed Speculative Intermittent Computation

This paper presents CoSpec, a new architecture/compiler co-design scheme that works for commodity in-order processors used in energy-harvesting systems. To achieve crash consistency without requiring unconventional architectural support, CoSpec leverages speculation assuming that power failure is not going to occur and thus holds all committed stores in a store buffer (SB), as if they were speculative, in case of mispeculation. CoSpec compiler first partitions a given program into a series of recoverable code regions with the SB size in mind, so that no region overflows the SB. When the program control reaches the end of each region, the speculation turns out to be successful, thus releasing all the buffered stores of the region to NVM. If power failure occurs during the execution of a region, all its speculative stores disappear in the volatile SB, i.e., they never affect program states in NVM. Consequently, the interrupted region can be restarted with consistent program states in the wake of power failure. To hide the latency of the SB release, i.e., essentially NVM writes, at each region boundary, CoSpec overlaps the NVM writes of the current region with the speculative execution of the next region. Such instruction level parallelism gives an illusion of out-of-order execution on top of the in-order processor, achieving a speedup of more than 1.2X when there is no power outage. Our experiments on a set of real energy harvesting traces with frequent outages demonstrate that CoSpec outperforms the state-of-the-art scheme by 1.8~3X on average.

==> src/problem.tex <==
%\subsection{Problem Definition}]
\subsection{Ultra Low Power Micro-architecture}
Despite of lower performance, prior works have mostly chosen "ultra-low power"
in-order processor architecture for power-hungry energy harvesting system
because it is more suitable than power-consuming and complex out-of-order processor
architecture~\footnote{ Some prior works suggested out-of-order processor or
even hybrid cores (in-order and out-of-order), however; they all assume strong
energy harvesting situations~\cite{ma2017spendthrift,ma2015architecture}.}.
Also, since power failures become the norm in energy-harvesting systems, their
processors should have byte-addressable nonvolatile memory (NVM) for the
efficient backup/recovery across the failures, e.g., TI's MSP430FR series of
microcontrollers (MCU) have already integrated in-order core with FRAM. 
\ignore{
Now, prior works targets in-order MCUs 
with FRAM-based main memory 
~\cite{WISP,WISPcam,MSP430FR5969,maeng2017alpaca,hicks2017clank,Chain,baghsorkhi2018automating,Chinchilla,dino,Ratchet,Wang_2012,Lui_2015,Xie_2015}.}
Now, \name targets MCUs with FRAM-based main memory and
conventional microarchitecture without cache as in prior
work~\cite{Ratchet,hicks2017clank,Wang_2012,Lui_2015,Xie_2015}.
Without volatile memory like caches, thanks to the simplicity, 
only data in a processor, i.e., registers, are transient
and will be lost on power outage; they need to be checkpointed for safe recovery.


\subsection{Crash Consistency}
Thanks to crash consistency recovery schemes for reliable
backup/recovery~\cite{maeng2017alpaca,Chain,baghsorkhi2018automating,Chinchilla,dino,Ratchet},
the system can intermittently backup/checkpoint data and restore them across
power failures without memory inconsistency issue. 
However, the recovery schemes may require user-intervention
and cause poor performance (50$\sim$400\% overhead) due to the limit of
static analysis~\cite{Clank}.

To lighten the overhead and eliminate additional burden to end-users, prior works have
suggested hardware solutions by using (1) voltage monitoring system~\cite{3us, Ambient,
Wang_2012,Lui_2015, ma2017incidental, hibernus2015,
balsamo2016hibernus++,jayakumar2014quickrecall} or
(2) idempotent detector~\cite{Clank} 






\ignore{
Obviously, because of the nature of in-order processor design and such a long NVM write latency, the prior works may cause poor performance. \ignore{
Unlike the prior works, \name enables out-of-order program execution on top of in-order processor for energy harvesting system. This paper will discuss about this in Section~\ref{sec:overview}.
}
Also, prior works require non-trivial hardware modification to address crash consistency issues for reliable intermittent computation: 
(1) voltage monitoring based checkpoint protocol or (2) idempotent detection logic with dynamic checkpoint mechanism.
\ignore{
Due to the possibility of checkpoint failure and potential memory inconsistency problem, e.g., 
power outages can happen during checkpointing, and the system may not
atomically update value in NVM resulting in incorrect recovery in the wake of power failure, prior works have suggested
}
\ignore{

all require
reliable energy guarantee to take full checkpoints to NVM. Incomplete
checkpoints can cause crash inconsistency issues, which causes inconsistent
values across different memory locations and cause erroneous re-execution.
These prior works rely on a variety of circuit-level techniques to guarantee
reliable energy to write complete checkpoints to NVM before the CPU shuts down
due to power outage. Below, we discuss the problems and overheads of these
circuit-level techniques. 
}
}
\subsubsection{Voltage Monitoring}
\label{sec:problem:buffer}
%Capacitors are commonly used as energy buffers in embedded systems ~\cite{chen2013stacked,wang2008determination}. When using the energy buffer, the systems do not boot until the buffer (capacitor) is fully charged as with commodity systems such as WISP~\cite{wisp5}.  
%An energy buffer helps to supply the required power when an electric component depends upon a specific amount of power. 
A popular model for energy-harvesting systems is to use a capacitor as an
energy buffer to accumulate harvested energy. For these energy-harvesting
systems, a common requirement among prior works ~\cite{3us, Ambient,
Wang_2012,Lui_2015, ma2017incidental, hibernus2015,
balsamo2016hibernus++,jayakumar2014quickrecall} is to use a voltage monitor to
ensure there is sufficient energy left in the capacitor to take a full
checkpoint; the voltage monitor alerts the CPU to take a checkpoint and power
down when the voltage monitor estimates that the capacitor only contains
sufficient energy for checkpointing and nothing else.  However, reliably
estimating whether there is only sufficient energy left in the capacitor to
take a checkpoint is difficult, as this requires predicting the future rate of
charge discharge. However, the capacitor can suffer from unstable  discharge
due to in-field aging problems such as cracking~\cite{capcrack,CapLeak}.
Increased discharge rate can lead the voltage monitor underestimate the future
rate of charge dissipation and, therefore, result in partial checkpointing.
While the voltage monitor may address the unpredictable discharge rate problem
by pessimistically overestimating the discharge rate, this  unnecessarily
increase checkpointing frequency, which reduces performance, energy efficiency,
and increases wear-out rate of the NVM.  Moreover, the energy buffer is
vulnerable to physical access
attack~\cite{cronin2018collaborative,cronin2017danger}, whereby the attackers
can shorten the capacitor or detach it from the device then inject malicious
voltage fluctuation into the target board. If so, attackers can maliciously
cause the voltage monitor to create partial checkpoints that lead to malicious
memory inconsistency problems ~\cite{cronin2018collaborative,cronin2017danger}.
Due to their ubiquitous nature, energy-harvesting devices are particularly
susceptible to physical attacks. 

%This urges the existing intermittent computation schemes to be robust against such security attacks.

\ignore{
The voltage monitor based checkpoint schemes~\cite{3us, Ambient, Wang_2012,Lui_2015, ma2017incidental, hibernus2015, balsamo2016hibernus++,jayakumar2014quickrecall} may not avoid
partial checkpoint because of energy buffer vulnerability/instability issues, 
and the voltage monitor excessively increases the system start-up voltage level
much higher incurring energy inefficiency. 
Also, the voltage monitor free design~\cite{hicks2017clank} causes unexpected
memory inconsistency issue due to faulty data dependent detector logic. 
In this section, this paper discusses about 
(1) energy buffer vulnerability/instability, (2) start-up voltage increment by 
voltage monitoring system, and (3) unexpected memory inconsistency issue from 
data dependent detection logic.
}

\ignore{
\subsection{Energy Buffer Vulnerability/Instability}
\label{sec:problem:buffer}
A capacitor as energy buffer is a common solution in embedded system 
area~\cite{chen2013stacked,wang2008determination}. 
At a high level, when an electric 
component depends upon a specific amount of power, the energy buffer 
is placed to 
provide required power. 
Energy harvesting systems use a capacitor as the energy buffer in the same way. By using the energy buffer, 
the systems do not boot until the buffer (capacitor) is fully charged as with commodity
systems such as WISP~\cite{wisp5}. In the wake of
each power outage, it is thus assured that the program can
make as much progress as the full energy buffer allows, even
if no additional energy is harvested.
To safely checkpoint voltage states to NVFF, the state-of-the-art, NVPs~\cite{3us}, require additional energy buffer. 
}

\ignore{
\paragraph{Energy Buffer Vulnerability}
Unfortunately, the energy buffer may be vulnerable by physical access attack~\cite{cronin2018collaborative,cronin2017danger}, e.g.,
attackers can shorten the capacitor or detach
it from the device then inject malicious voltage fluctuation into
the target board. If so, attackers can finally make the system 
worn out or partially checkpoint resulting in memory inconsistency
~\cite{cronin2018collaborative,cronin2017danger}.
}
\ignore{
\paragraph{Energy Buffer Instability}
The capacitor can suffer from stability issues such 
as excessive
leakage or crack leading to reduced 
capacitance~\cite{capcrack,CapLeak}. Cracked capacitor may also cause partial checkpointing, then it finally incurs memory inconsistency problems. This urges the existing intermittent computation schemes to be robust against such
security attacks.
}

%Because of these issues, \name approaches to energy-buffer-free hardware design in a way of the prior work~\cite{wang2016storage,lee2015powering}. 


%indicates the state-of-the-arts cause 
%non-trivial unreliability problems.

%such as start-up voltage increment, 
%energy buffer vulnerability/stability issues, non-deterministic path problem, 
%and unexpected memory inconsistency. 
%\subsection{Wake-up Voltage Increment}

To address the 
energy buffer issues and inaccurate timing error 
of voltage monitoring system, 
prior works suggest energy-storage free design~\cite{wang2016storage,lee2015powering} and advanced
voltage detection logic~\cite{su2017ferroelectric}.
However, these schemes ended up increasing
wake-up/back-up voltage level for safe recovery and checkpoint by almost 2$\sim$3X comparing to the previous works~\cite{3us, Ambient};
the system could have started at about 1$\sim$1.8V~\cite{3us,
Ambient,msp430manual}, however; the state-of-the-art set the threshold up high
as 2.7$\sim$3V~\cite{su2017ferroelectric,wang2016storage,lee2015powering}
~\footnote{
Prior work~\cite{su2017ferroelectric} found that the
backup/recovery controller may make a wrong reboot decision, which may cause
potential data corruption problem, due to the cold-start
voltage spark or an unexpected glitch.}. 
Consequently, they waste
hard-won energy for nothing until the sufficient voltage is
provided to wake up the system.


\ignore{
Prior works~\cite{3us, Ambient, Wang_2012,Lui_2015, ma2017incidental, hibernus2015, balsamo2016hibernus++,jayakumar2014quickrecall} have approached the voltage 
monitoring system to checkpoint before the impending power outage.
Figure~\ref{fig:NVPmodel} describes one of the state-of-the-arts, NVP model~\cite{3us, Ambient, Wang_2012,Lui_2015, ma2017incidental}, in detail.
\begin{figure}[!h]
\centering
\centerline{\includegraphics[width=\columnwidth, angle=0]{fig/nvpdesign.pdf}}
\centering
\caption{NVP model}
\label{fig:NVPmodel}
\end{figure}
}

%Higher voltage-required components such as voltage comparator and voltage reference
%are inevitable in their design.



%The components excessively limit the system start-up voltage threshold to be 
%much high, e.g., the system could have started at about 1$\sim$1.8V~\cite{3us, Ambient,msp430manual},
%however; it has to set the threshold up high, e.g., 
%2.7$\sim$3V~\cite{su2017ferroelectric,wang2016storage,lee2015powering}
%because of the components~\cite{Comparator,su2017ferroelectric}.




\ignore{
To monitor the input voltage fluctuation with/without energy storage,
the system should have
equipped with higher voltage-required  components such as
voltage comparator and voltage reference, e.g.,
the voltage monitor logic basically requires the components to compare input 
voltage with the reference voltage, then it can determine whether 
the controller should wake up or sleep the system.
These components have to be stable as the first prioritized task 
in the system booting process, otherwise; they may make 
a wrong reboot decision 
resulting in
potential memory inconsistency problem due to 
cold-start voltage spark~\cite{su2017ferroelectric}.}

\ignore{
Unlike the prior works~\cite{wang2016storage,lee2015powering,su2017ferroelectric}, %\name is 
%not required to equip with such redundant components, i.e.,
\name is voltage monitor free for power-hungry energy harvesting system design
without considering the wrong reboot decision. 
Even further, \name can suggest undervolting execution at the cost of timing error 
penalty~\cite{menon2012igpu}. 
%This paper will describes its design in Section~\ref{sec:overview}
}
\subsubsection{Voltage Monitor Free Design}
Prior work, Clank~\cite{hicks2017clank}, suggested the
voltage-monitor-free design by leveraging idempotent processing in hardware
level.  Clank tracks all memory accesses at run-time with several memory
buffers: write-back, load-first, write-first, and address buffers.  By using
load-first and store-first buffers, Clank monitors anti-dependent load-store
pairs. If it found, the system checkpoints and drains the write-back buffer to
non-volatile scratchpad then copies the drained data to NVMM.  Also, when the
buffer becomes full, Clank exceptionally checkpoints and drains the buffer in
the same way of idempotent detection case.  Unfortunately, Clank requires
non-trivial hardware modification; non-volatile scratchpad does not even exist
in real-world~\footnote{The scheme may adapt NVSRAM, then it has the same
problem with the voltage monitoring system (not voltage monitor free
anymore).}.  In addition, since the scheme may cause frequent checkpoints
at each anti-dependent pair and buffer-overflow, it
results in poor performance (the paper says 20\% performance overhead with
non-volatile scratchpad).


In contrast, \name is low-cost architecture/compiler co-design enabling reliable
out-of-order execution for high performance intermittent computation;
\name addressses crash consistency without hardware modification, and it is still
able to achieve high performance intermittent computation.

\ignore{
From these challenges,
this paper mainly asks questions as following:
\begin{compactitem}
\item How to improve the performance which may be limited by in-order processor design?
\item{How to eliminate non-trivial hardware modification?}
\item{How to cost-efficiently address the crash consistency issue?}

\end{compactitem}

}


\ignore{
the double buffering NVM writes may cause
poor performance due to possibly frequent checkpoints and double buffering
scheme which comes along doubled persistent writes, e.g., their scheme stalls
at each checkpoint until their NVM writes are completely saved into the final
memory location. 
}

\ignore{, e.g., their scheme first holds persistent stores in
	the write-back buffer, then releases them to non-volatile buffer, and then
	finally copies the buffered data to original non-volatile memory location.
	Unfortunately, the scheme may cause significant
performance overhead and redundant hardware modification cost.}
%since the scheme heavily relies on inaccurate detector, it may not address the memory inconsistency problem.

%\subsubsubsection{Performance Overhead}
%\subsection{Non-deterministic Path}
%Due to the simple design for energy harvesting system,
\ignore{
First, Clank checkpoints when its write-back buffer is full. If the buffer becomes full, the system would checkpoint committing buffered stores to non-volatile scratchpad then copies them again to non-volatile main memory.
Due to this double buffering protocol coming along doubled persistent writes, Clank causes considerable performance overhead. According to their work~\cite{Clank}, the scheme causes more than 20\% overhead at the similar buffer size of \name.

In addition, due to the non-deterministic path issue,
Clank aggressively checkpoints at certain case. 
%due to
%optimistically optimized write back buffer.
%by allowing systems to overwrite data taking a different path
%due to random function predicates.
Figure~\ref{fig:nondeter} describes how non-deterministic path issue 
can occur.
Supposedly, the system accesses to a random function predicate in
the first basic block on the top, then flows to the false branch
on the right hand side and stores 
new data (r10) to memory address (\&mem[100]).
If a power outage occurs after the memory store, 
the system would restart at the last checkpointed boundary with
already updated data in the memory (\&mem[100]) in the wake of power failure.
Since the random function predicate allows the system to take
a different path (left hand side) after the recovery, 
the system would possibly load the overwritten data from the 
memory resulting in memory inconsistency problem.
To address this potential memory inconsistency, Clank should checkpoint before the store, and it may causes additional checkpoint overhead.

%This problem may not occur software schemes~\cite{} because they may cut

%To address this issue, \name suggests store buffer design by holding committed stores
%then atomically releasing or discarding them.

\begin{figure}[!h]
\centering
\centerline{\includegraphics[width=\columnwidth, angle=0]{fig/nondet.pdf}}
\centering
\caption{Non-deterministic Path Scenario. In this figure, the system may first
	take the false path (right side), 
then it has a power outage problem.
After recovery, it goes through the true path (left side) later because of different random function return value.}
\label{fig:nondeter}
\end{figure}


%\subsubsection{Hardware Cost}
Second, Clank requires additional hardware support: a idempotent violation detector logic, a non-volatile 
scratchpad, and four extra buffers which are write-back, load-first, write-first, and address buffers. 
This hardware 
modification cost can be saved by following \name architecture. 
}


\ignore{
Also, the idempotent violation detection logic may carefully consider
alignment issue of memory access instructions, e.g., if the system first 
reads 4 bytes from memory address (\&mem[1000]) then stores 1 byte data at 
different memory address (\&mem[1001]), the detector should raise an alarm.
%, i.e., the load and store are data dependent.  
Unlike the prior work, \name is low-cost lightweight architecture/compiler co-design leveraging only current commodity hardware components.
}

\ignore{
Unfortunately, the detector determines they are 
not an anti-dependent pair because their memory addresses are 
different. This memory alignment problem may not be occurred in some 
types of architectures, however; MSP430 and RISC V architectures may 
cause the problem.
}
\ignore{
\subsubsection{Memory Alignment Issue}
The data dependent detector of Clank tracks load and store instructions 
without considering memory alignment issue. 
For example, the system first reads 4 bytes from memory address (\&mem[1000]), then it saves 1 byte data at different memory address (\&mem[1001]).
%, i.e., the load and store are data dependent.  
Unfortunately, the detector determines they are 
not an anti-dependent pair because their memory addresses are 
different. This memory alignment problem may not be occurred in some 
types of architectures, however; MSP430 and RISC V architectures may 
cause the problem.
}
%To address these issues, \name approaches precise store buffer based truly
%recoverable program execution by leveraging compiler support.
%This problem indicates that existing intermittent computation schemes
%~\cite{Ratchet,dino,Chain,colin2018termination,Alpaca,hicks2017clank}
%demands secure hardware support or users' expertise.

%and this paper approaches to robust
%compiler-cooperated system architecture. 

\ignore{
\subsection{Energy Buffer Vulnerability}
A capacitor as energy buffer is a common solution in embedded system 
area~\cite{chen2013stacked,wang2008determination}. 
At a high level, when an electric 
component depends upon a specific amount of power, the energy buffer 
is placed to 
provide required power. 
Energy harvesting systems use a capacitor as the energy buffer in the same way. By using the energy buffer, 
the systems do not boot until the buffer (capacitor) is fully charged as with commodity
systems such as WISP~\cite{wisp5}. In the wake of
each power outage, it is thus assured that the program can
make as much progress as the full energy buffer allows, even
if no additional energy is harvested.
To safely checkpoint voltage states to NVFF, the state-of-the-art, NVPs~\cite{3us}, require additional energy buffer. 

However, the energy buffer may be vulnerable by physical access attack~\cite{cronin2018collaborative,cronin2017danger}, e.g.,
attackers can shorten the capacitor or detach
it from the device then inject malicious voltage fluctuation into
the target board. If so, attackers can finally make the system 
worn out~\cite{cronin2017danger}. 
In addition, the capacitor can suffer from stability issues such 
as excessive
leakage or crack leading to reduced 
capacitance~\cite{capcrack,CapLeak}. Cracked capacitor may cause partial checkpointing, then it finally incurs memory inconsistency problems. This urges the existing intermittent computation schemes to be robust against such
security attacks.
}

